DIVERSIFY: A General Framework for Time Series Out-of-distribution Detection and Generalization

Time series remains one of the most challenging modalities in machine learning research. The out-of-distribution (OOD) detection and generalization on time series tend to suffer due to its non-stationary property, i.e., the distribution changes over time. The dynamic distributions inside time series pose great challenges to existing algorithms to identify invariant distributions since they mainly focus on the scenario where the domain information is given as prior knowledge. In this paper, we attempt to exploit subdomains within a whole dataset to counteract issues induced by non-stationary for generalized representation learning. We propose DIVERSIFY, a general framework, for OOD detection and generalization on dynamic distributions of time series. DIVERSIFY takes an iterative process: it first obtains the "worst-case" latent distribution scenario via adversarial training, then reduces the gap between these latent distributions. We implement DIVERSIFY via combining existing OOD detection methods according to either extracted features or outputs of models for detection while we also directly utilize outputs for classification. In addition, theoretical insights illustrate that DIVERSIFY is theoretically supported. Extensive experiments are conducted on seven datasets with different OOD settings across gesture recognition, speech commands recognition, wearable stress and affect detection, and sensor-based human activity recognition. Qualitative and quantitative results demonstrate that DIVERSIFY learns more generalized features and significantly outperforms other baselines.

==> tab/tb-emg-diff.tex <==
\begin{table*}[!t]
\caption{Results on EMG dataset with different model sizes.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|lllll|lllll|lllll}
\toprule
Model Size & \multicolumn{5}{c|}{Small}                                                     & \multicolumn{5}{c|}{Medium}                                                    & \multicolumn{5}{c}{Large}                                                     \\
Target     & 0             & 1             & 2             & 3             & AVG           & 0             & 1             & 2             & 3             & AVG           & 0             & 1             & 2             & 3             & AVG           \\ \midrule
ERM        & 56.6          & 65.7          & 65.3          & 61.8          & 62.3          & 62.6          & 69.9          & 67.9          & 69.3          & 67.4          & 61.2          & 78.8    & 68.8          & 64.6          & 68.4          \\
DANN       & 65.3          & 69.3          & 63.6          & 62.9          & 65.3          & 62.9          & 70.0          & 66.5          & 68.2          & 66.9          & 63.0          & 72.7          & 69.4          & 68.5          & 68.4          \\
CORAL      & \underline{66.9}    & 74.9          & 70.8          & \underline{73.2}    & \underline{71.4}    & 66.4          & 74.6          & 71.4          & \underline{74.2}    & 71.7          & \underline{67.7}    & 77.0          & 72.7          & 71.8          & 72.3          \\
Mixup      & 56.8          & 61.0          & 68.1          & 67.2          & 63.2          & 60.7          & 69.9          & 70.5          & 68.2          & 67.3          & 66.3          & \underline{81.1}          & 71.2          & 69.6          & 72.0          \\
GroupDRO   & 64.9          & \underline{75.0}    & \underline{71.6}    & 69.1          & 70.1          & 67.6          & \underline{77.5}    & \underline{73.7}    & 72.5          & \underline{72.8}    & 66.3          & 79.3          & \underline{74.9}    & 71.3          & \underline{73.0}    \\
RSC        & 62.7          & 73.2          & 67.6          & 64.0          & 66.9          & \underline{70.1}    & 74.6          & 72.4          & 71.9          & 72.2          & 65.1          & 76.8          & 72.2          & 67.7          & 70.4          \\
ANDMask    & 62.4          & 66.0          & 66.3          & 65.6          & 65.1          & 66.6          & 69.1          & 71.4          & 68.9          & 69.0          & 65.7          & 78.1          & 72.1          & \underline{71.9}    & 71.9          \\ 
DIVERSIFY  & \textbf{69.8} & \textbf{77.3} & \textbf{74.4} & \textbf{74.4} & \textbf{74.0} & \textbf{71.7} & \textbf{82.4} & \textbf{76.9} & \textbf{77.3} & \textbf{77.1} & \textbf{72.0} & \textbf{86.6} & \textbf{78.5} & \textbf{78.9} & \textbf{79.0}\\ \bottomrule
\end{tabular}}

\label{tab:my-table-difmodelsize}
\end{table*}

==> tab/tb-emg.tex <==
\begin{table}[htbp]
% \vspace{-.1in}
\centering
\caption{Results on EMG dataset. ``Target'' $0 \sim 4$ denotes unseen test distribution that is only for testing.}
% \vspace{.1in}
\label{tab:my-table-EMG}
\resizebox{.35\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
Target   & 0    & 1    & 2    & 3    & AVG  \\ \midrule
ERM      & 62.6 & 69.9 & 67.9 & 69.3 & 67.4 \\  
DANN     & 62.9 & 70.0 & 66.5 & 68.2 & 66.9 \\ 
CORAL    & 66.4 & 74.6 & 71.4 & 74.2 & 71.7 \\ 
Mixup    & 60.7 & 69.9 & 70.5 & 68.2 & 67.3 \\
GroupDRO & 67.6 & \underline{77.4} & \underline{73.7} & 72.5 & 72.8 \\ 
RSC      & \underline{70.1} & 74.6 & 72.4 & 71.9 & 72.2 \\ 
ANDMask  & 66.5 & 69.1 & 71.4 & 68.9 & 69.0 \\
AdaRNN &68.8 &81.1 &75.3 &\textbf{78.1} &\underline{75.8}\\
\method & \textbf{71.7} & \textbf{82.4} & \textbf{76.9} & \underline{77.3} & \textbf{77.1} \\ \bottomrule
\end{tabular}
}
% \vspace{-.1in}
\end{table}

==> tab1/emg-odin.tex <==
\begin{table}[htbp]
\centering
\caption{AUROC and AUPR  on EMG and WESAD with ODIN. \textbf{Bold} means the best. \wjd{This can be plot with figure 12 and leave the detailed results in appendix. Then merge fig. 13 with 12 so one figure has 5 subfigures.}}
\label{tab1-odin}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{clllllllllll}
\toprule
\multicolumn{1}{l}{Dataset} & Metrics                     & \multicolumn{5}{c}{AUROC}                                                          & \multicolumn{5}{c}{AUPR}                                                           \\
\multirow{7}{*}{EMG}        & Targets                     & 0              & 1              & 2              & 3              & AVG            & 0              & 1              & 2              & 3              & AVG            \\ \midrule
                            & ERM-ODIN                    & 73.80          & 65.60          & 54.58          & 47.22          & 60.30          & 92.85          & 89.43          & 86.46          & 84.23          & 88.24          \\
                            & CORAL-ODIN                  & \textbf{74.18} & 71.09          & 73.80          & 43.80          & 65.72          & \textbf{93.51} & 92.33          & 93.69          & 81.68          & 90.30          \\
                            & DANN-ODIN                   & 64.65          & 73.59          & 76.63          & 69.29          & 71.04          & 89.73          & 92.21          & 93.78          & 89.79          & 91.38          \\
                            & GroupDRO-ODIN               & 65.70          & 75.10          & 71.07          & \textbf{72.48} & 71.09          & 89.74          & 93.15          & 92.36          & 91.69          & 91.74          \\
                            & ANDMask-ODIN                & 52.81          & 80.14          & 69.68          & 26.97          & 57.40          & 85.38          & 94.20          & 92.06          & 74.88          & 86.63          \\
                            & \method-ODIN & 65.10          & \textbf{84.52} & \textbf{80.02} & 72.21          & \textbf{75.46} & 90.75          & \textbf{95.90} & \textbf{95.36} & \textbf{92.44} & \textbf{93.61} \\ 
                            \midrule
\multirow{7}{*}{WESAD}      & Targets                     & 0              & 1              & 2              & 3              & AVG            & 0              & 1              & 2              & 3              & AVG            \\ \midrule
                            & ERM-ODIN                    & 67.63          & 54.72          & 37.21          & 34.29          & 48.46          & 87.59          & 77.99          & 76.22          & 71.93          & 78.43          \\
                            & CORAL-ODIN                  & 72.56          & 61.58          & 60.10          & \textbf{94.34} & 72.15          & 90.63          & 78.26          & 81.28          & \textbf{98.10} & 87.07          \\
                            & DANN-ODIN                   & 60.21          & 60.06          & 57.64          & 64.44          & 60.59          & 87.19          & 77.08          & 83.03          & 88.39          & 83.92          \\
                            & GroupDRO-ODIN               & 61.93          & 54.73          & 52.27          & 90.25          & 64.80          & 87.58          & 79.93          & 80.92          & 96.95          & 86.35          \\
                            & ANDMask-ODIN                & 60.71          & 51.79          & 35.61          & 73.52          & 55.41          & 86.91          & 73.70          & 67.58          & 90.58          & 79.69          \\
                            & \method-ODIN & \textbf{85.98} & \textbf{66.00} & \textbf{71.47} & 88.59          & \textbf{78.01} & \textbf{94.25} & \textbf{88.22} & \textbf{89.73} & 96.50          & \textbf{92.18} \\ \bottomrule
\end{tabular}}
\end{table}
